Millions of Little Minions: Using Packets for Low Latency Network Programming and Visibility (Extended Version)

This paper presents a practical approach to rapidly introduce new dataplane functionality into networks: End-hosts embed tiny programs into packets to actively query and manipulate a network's internal state. We show how this "tiny packet program" (TPP) interface gives end-hosts unprecedented visibility into network behavior, enabling them to work with the network to achieve a common goal. Our design leverages what each component does best: (a) switches forward and execute tiny packet programs (at most 5 instructions) at line rate, and (b) end-hosts perform arbitrary computation on network state, which are easy to evolve. Using a hardware prototype on a NetFPGA, we show our design is feasible, at a reasonable cost. By implementing three different research proposals, we show that TPPs are also useful. And finally, we present an architecture in which they can be made secure.

==> Makefile <==
TARGET=tpp
BIBTEX := bibtex
OS := $(shell uname)
SOURCES=$(TARGET).tex $(wildcard *.tex) $(wildcard images/*)\
    $(TARGET).bib

ifeq ($(OS), Darwin)
all: $(TARGET)-extended.pdf
else
all: $(TARGET).pdf
endif

ifeq ($(OS), Darwin)
$(TARGET)-extended.pdf: $(SOURCES)
	latexmk -pdf $(TARGET)-extended.tex
$(TARGET).pdf: $(SOURCES)
#	pdflatex $(TARGET).tex
#	$(BIBTEX) $(TARGET)
#	pdflatex $(TARGET)
#	pdflatex $(TARGET)
#	grep undef *.log || true
	latexmk -pdf $(TARGET).tex
	if [ -d ~/Dropbox/tpp-sigcomm14 ]; then cp $(TARGET).pdf ~/Dropbox/tpp-sigcomm14/tpp.pdf; fi
else
$(TARGET).pdf: $(SOURCES)
	latexmk -pdf -interaction=nonstopmode -halt-on-error \
			-file-line-error $(TARGET).tex
endif

pdf: $(TARGET).pdf
	xpdf $(TARGET).pdf

view: $(TARGET).pdf
	open $(TARGET).pdf

clean:
	latexmk -quiet -C $(TARGET).tex
	rm -f `cat .gitignore` .*~
	@extraneous=`git ls-files -o`; if test -n "$$extraneous"; then \
		echo WARNING:  The following files are not in git:; \
		printf "        %s\n" $$extraneous; \
		exit 1; \
	fi
#	rm -f *.aux *.log *.out *.bbl *.blg *~ *.bak *.synctex.gz $(TARGET).pdf


==> background.tex <==

%We use the term dataplane to refer to the part of a switch that is
%involved in processing {\em every packet}.  In a hardware switch, it
%is the ASIC.  However, our design principles equally apply to high
%performance software switches (e.g., in virtualized datacenters or a
%wireless router), where the datapath is the kernel module (e.g.,
%OpenVSwitch or the Linux Bridge).
%We use the term
%control plane to refer to the control software that configures how the
%dataplane should route packets.  The control plane could be a BGP
%software instances running on the switch CPU, or an
%OpenFlow~\cite{mckeown2008openflow} controller.

%% The modules are connected through registers that contain packet data.
%% The internal ASIC clock that drives the hardware logic transfers data
%% from one module to another.  It is important to note that the hardware
%% modules are pipelined, so processing happens (mostly) in parallel.
%% For instance, the header parser might take a few cycles to decode
%% packet data, during which additional packet data is queued in a
%% temporary buffer.

\begin{comment}
Such programmability is accessible today primarily through the {\em
  control plane} through protocols such as OpenFlow.  Control plane
access is typically slow due to two main reasons.  First, the control
plane introduces multiple layers of abstraction that add latency.  For
instance, an OpenFlow controller sends a flow-modification message
through a TCP channel, which is then interpreted by an OpenFlow Agent
running on the switch.  The OpenFlow agent compiles and optimizes this
flow entry, and sends a command to the ASIC to insert a new entry into
one of its tables.  Second, the resources available on the switch are
typically limited in terms of processing and memory.  This second
reason may not be fundamental in nature, and in
\S\ref{sec:discussion}, we discuss how an improved switch control
agent could be used to incrementally deploy our scheme.

For many tasks such as routing and traffic engineering, such slow
access is typically sufficient.\footnote{However, it does not preclude
  proposals from getting around slow control plane convergence times
  through dataplane mechanisms~\cite{liu2013ensuring}.} However,
congestion control and network measurement require real time access to
network state to operate effectively.  For instance, congestion
control typically operates at timescales of a few round-trip times,
which can be as low as a few microseconds in the datacenter.  Network
measurement tasks, such as identifying heavy hitters in traffic in
real time, require few simple per-packet operations that operate in
the dataplane.  Thus, the control plane is ill-suited for tasks such
as congestion control and measurement, which are undisputedly critical
for a network's operation.  This observation motivates our approach to
accessing network state through the dataplane.

\vimal{Maybe move this to related work.} It is worth pointing out that
there have been numerous to expose switch statistics through the
dataplane, particularly to improve congestion management and network
monitoring.  A popular example is Explicit Congestion Notification
(ECN) in which a router stamps a bit in the IP header whenever the
egress queue occupancy exceeds a configurable threshold.  Another
example is IP Record Route, an IP option that enables routers insert
the interface IP address onto the packet.  This option has been used
in clever ways~\cite{katz2010reverse} to help operators diagnose
faulty network routes.
\end{comment}

